Analysing Austrian Parliamentary Speeches by Predicting Party Affiliations

This paper examines speech characteristics of the Austrian National Council members (CMs). We introduce analysis methodology based on a fine-tuned BERT-Model which assigns to every speech a probability distribution over Austrian parties. These are then aggregated at the speaker and party level. We perform an extensive evaluation to ensure the quality of the generated distributions prior to further analysis. Instead of considering mis-assignments of predicted parties as a performance issue, we leverage them to derive insights about the CMs and political developments. Our findings show that parties that govern together become more similar in their speech characteristics, while, analogously, parties that are in opposition move further away from governing parties. Moreover, CMs who switch party usually adapt their speech characteristics only after the switch occurs. Finally, we publicly release a data set containing party affiliation predictions for the speeches of the Austrian National Council from 1996 to 2018.

==> relatedworkshort.tex <==
\section{Related Work}
The introduction of BERT \cite{devlin2019bertpretrainingdeepbidirectional} and subsequent evaluations against alternative classifiers \cite{Garrido_Merchan_2023} have demonstrated the effectiveness of modern text classification approaches. While generative LLMs have been explored for tasks like elite polarization detection in the European Parliament \cite{iakovlev2025elitepolarizationeuropeanparliamentary}, recent comparisons show that fine-tuned BERT models often outperform prompted LLMs in text classification, particularly when contextual knowledge is required \cite{vajjala2025textclassificationllmera,zhang-etal-2025-bert-like}.

Early work by Gerrish and Blei \cite{gerrish2011predicting} developed predictive models linking legislative sentiment to legislative text to predict voting patterns. In the domain of political discourse, Reinig et al. \cite{reinig-etal-2024-politics} identified rhetorical differences between government and opposition through speech act analysis, while Pätz et al. \cite{pätz2025analyzinggermanparliamentaryspeeches} emphasized the need for specialized embeddings to capture political speech nuances. Navarretta and Hansen \cite{navarretta2024government} used a pre-trained Danish BERT model to classify speeches by parties in government, opposition, or “other” roles, achieving F1-scores of 0.64 (3-class) and 0.77 (binary), and Abercrombie and Batista-Navarro \cite{abercrombie2022policy} identified policy preferences and speech sentiment in UK parliamentary debates using transformer-based models.

Other work has applied these techniques to different tasks. The GREEK-BERT model was fine-tuned for party prediction in both binary and multiclass tasks \cite{10345868}. In the Australian Parliament, stance classification compared BERT and tf-idf, with tf-idf outperforming BERT in prediction performance and computational efficiency while offering greater transparency \cite{repec:spr:jcsosc:v:8:y:2025:i:2:d:10.1007_s42001-025-00366-y}. Timoneda and Vera \cite{doi:10.1086/730737} evaluated transformer models, highlighting the need for balanced training data—a particular challenge for small parties with limited speeches. Reinig et al. \cite{reinig-etal-2024-politics} also annotated speeches by speech act using both tf-idf with SVM and fine-tuned BERT, finding that parties adopt different rhetorical strategies in opposition versus government, aligning with our findings.

The ParlSpeech V2 dataset \cite{DVN/L4OAKN_2020}, containing full-text corpora of 6.3 million parliamentary speeches from nine democracies, serves as the foundation for this paper. Fišer and Skubic \cite{skubic2024parliamentary} provide a literature review on parliamentary discourse research in political science, showing how parliamentary corpora can be integrated into political science research. 

In contrast to prior work, we use fine-tuned BERT to predict probabilistic party affiliations for each speech, aggregating these to analyze linguistic proximity between parties and politicians over time. Unlike previous studies, we leverage misclassifications to reveal political dynamics, such as coalition convergence and opposition divergence. Additionally, we publicly release a dataset of party affiliation predictions for Austrian parliamentary speeches from 1996 to 2018.
